Evaluating Built-in ECC of FPGA on-chip Memories for the Mitigation of Undervolting Faults

Voltage underscaling below the nominal level is an effective solution for improving energy efficiency in digital circuits, e.g., Field Programmable Gate Arrays (FPGAs). However, further undervolting below a safe voltage level and without accompanying frequency scaling leads to timing related faults, potentially undermining the energy savings. Through experimental voltage underscaling studies on commercial FPGAs, we observed that the rate of these faults exponentially increases for on-chip memories, or Block RAMs (BRAMs). To mitigate these faults, we evaluated the efficiency of the built-in Error-Correction Code (ECC) and observed that more than 90% of the faults are correctable and further 7% are detectable (but not correctable). This efficiency is the result of the single-bit type of these faults, which are then effectively covered by the Single-Error Correction and Double-Error Detection (SECDED) design of the built-in ECC. Finally, motivated by the above experimental observations, we evaluated an FPGA-based Neural Network (NN) accelerator under low-voltage operations, while built-in ECC is leveraged to mitigate undervolting faults and thus, prevent NN significant accuracy loss. In consequence, we achieve 40% of the BRAM power saving through undervolting below the minimum safe voltage level, with a negligible NN accuracy loss, thanks to the substantial fault coverage by the built-in ECC.

==> Camera-Ready-5pages_arXiv/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


***************************** Subdirectories ******************************

bibtex   - The IEEEtran BibTeX style package.

extras   - Supplementary material that may be of interest.

testflow - The testflow diagnostic suite for verifying PS/PDF output.

tools    - The IEEEtrantools.sty package which provides several commands
           from the IEEEtran.cls file for use with other LaTeX classes.


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex,
                   bare_jrnl.tex, bare_jrnl_comsoc.tex,
                   bare_jrnl_compsoc.tex, bare_jrnl_transmag.tex
***************************************************************************


==> Camera-Ready-5pages_arXiv/chapters/10-overallbehaviour.tex <==
\section{Overall Behavior on BRAM Undervolting}
Our experiments on undervolting BRAMs below nominal level, $V_{nom}= 1V$, demonstrate two thresholds. \textit{First}, a voltage guardband, $V_{min}$, that separates the fault-free and faulty regions. \textit{Second}, $V_{crash}$ that is the lowest level of the voltage that our design practically operates, below that FPGA fails. In our test environment and for both tested platforms, $V_{nom}= 1V$ due to the factory settings, whereas $V_{min}= 0.61V$ and $V_{crash}= 0.54V$, obtained through our experiments. Note that repeating these tests in more noisy and harsh environments, worst case scenarios, can cause observable faults above 0.61V, as well; however, our tests are performed under normal environmental conditions. Also, due to our experiments with various Xilinx FPGAs at 28nm technology, we posit that $V_{crash}= 0.54V$ is strictly set by the factory to prevent device damage in extremely low voltages.%



\begin{figure}
  \includegraphics[width=0.9\linewidth]{./images/85.png}
  \caption{BRAM Power above $V_{min}=0.61V$ in the voltage guardband region (no observable fault).}
  \label{fig:breakdown}
\end{figure}

\begin{figure}[!t]
\centering
\subfloat[VC707]{\includegraphics[width=0.9\linewidth]{./images/86.png}%
\label{subfig:major707}}
\hfill
\subfloat[KC705]{\includegraphics[width=0.9\linewidth]{./images/87.png}%
\label{subfig:major705}}
\caption{BRAM Power and Fault Rate Behavior, undervolting below $V_{min}=0.61V$ until $V_{crash}=0.54V$.}
\label{fig:cop}
\end{figure}

When $V_{CCBRAM} >= V_{min}$, no observable faults occur. When $V_{CCBRAM}= V_{min}= 0.61V$ we observed significant BRAM power savings over $V_{nom}= 1V$, more than an order of magnitude for both platforms, without incurring any reliability degradation, as shown in Fig. \ref{fig:breakdown}. Further lowering $V_{CCBRAM}$ below $V_{min}$ the fault rate exponentially increases, while the power consumption is reduced, as summarized in Fig. \ref{fig:cop}. %
As can be seen, both power consumption and reduction are less in KC705 than VC707, which is the consequence of having relatively less BRAMs and also the inherent power optimizations adopted for KC705 by the vendor.



==> Camera-Ready-5pages_arXiv/chapters/13-further.tex <==
\section{Summary and Further Discussion}
In this section, first, we summarize our key findings and later on, propose two more experimental observations of undervolting faults behavior that can be directly used in the design of customized and effective mitigation techniques. 

\subsection{Discussion on our Findings on Power and Reliability}
We summarize our findings on the power and reliability trade-off in low-voltage FPGAs, as follows:

\textit{-- Power:} Our experimental results on real hardware identified a significant potential in commercial FPGAs to operate in low-voltage regimes below the nominal level and in turn, to work in ultra-low-power modes. For an NN case study, we show the BRAMs power savings of more than an order of magnitude by voltage lowering until $V_{min}$ and a further 40\% below $V_{min}$, which in turn delivers 24.1\% total on-chip power reduction. Undevolting other power-hungry components of the accelerator, such as off-chip DDR-3 can potentially lead to further power savings gain, as it is evaluated to be 10.5\% on DDR-3 \cite{Chang2017}. %

\textit{-- Reliability:} Although, we observe that in FPGA-based BRAMs the fault rate below $V_{min}$ increases exponentially, they can be adequately mitigated using the built-in ECC, according to the behavior of these faults. The overhead of this ECC is not significant; however, for large word-width more efficient methods can be deployed. 

\begin{figure}
	\centering
  \includegraphics[width=\linewidth]{./images/203.png}
  \caption{Data Pattern Effects.}
  \label{subfig:pattern}
\end{figure}

\subsection{Discussion on the Further Observations: Proposals for Customized ECC in Low-voltage Regions}
We experimentally observe that the built-in ECC has a good capability to cover undervolting faults; however, it is power-optimized only for wide enough word-widths, as discussed in Section II.B. In this section, we describe two major experimental observations of the behavior of the undervolting faults, which can be potentially considered to build customized low-overhead ECC mechanisms.%
  
\begin{enumerate}
\item The vast majority of observed faults are "1" to "0" bit-flips, on average 99.9\%. This observation can be considered in a simplified ECC to deal with only "1" to "0" bit-flips. We verify this observation by repeating experiments on different data patterns on original size BRAMs. As shown in Fig. \ref{subfig:pattern}, the fault rate is proportional to the number of "1" bits; for example, with pattern= 16'hFFFF the fault rate is almost double than pattern= 16'hAAAA, and with pattern= 16'h0000 few faults are observed. In the same line, we did not observe any meaningful correlation in the various permutations of "0" and "1" in the data pattern; for instance, the fault rate of pattern= 16'hAAAA, 16'h5555, and a random pattern are almost the same. %
\item As earlier noted, BRAMs are composed of rows (1024 with the original size) and columns (18 with the original size). We experimentally observe that undervolting faults mostly manifest in a few certain columns within BRAMs. In other words, for each faulty BRAM, a few (one or two) most vulnerable column of bitcells exist, as illustrated in Fig. \ref{subfig:bram}. Fig. \ref{subfig:variability} shows the number of most vulnerable columns within faulty BRAMs. As can be seen, more than 80\% of faults occur in a single column, 17\% in two columns, and so on. However, these most vulnerable columns do not occur in the same column indexes, for different BRAMs. Due to this observation, we believe that column-based ECC can have a significant efficiency to mitigate these faults, with relatively lower power and area cost. %
\end{enumerate}
 



\begin{figure}[!t]
\centering
\subfloat[Illustration.]{\includegraphics[width=0.8\linewidth]{./images/BRAM2.pdf}%
\label{subfig:bram}}
\hfill
\subfloat[Statistical experimental results.]{\includegraphics[width=\linewidth]{./images/70.png}%
\label{subfig:variability}}
\caption{Within BRAM fault distribution, column-wise.}
\label{fig:further}
\end{figure}

==> Camera-Ready-5pages_arXiv/chapters/2-introduction.tex <==
\section{Introduction}

The power and energy efficiency of Field Programmable Gate Arrays (FPGAs) is estimated to be up to 20X less than Application Specific Integrated Circuits (ASICs) \cite{Zuchowski2002}. To alleviate this issue of FPGAs, many compiler-, architecture-, and circuit-level techniques have been proposed, in both academic research \cite{Sun2010}, \cite{Jamieson2009} and industry \cite{altera}, \cite{xilinx}. Among them, a very effective approach is undervolting, which can directly deliver static and dynamic power savings. Supply voltage is naturally scaled down with technology node evolution. For instance, for Xilinx device generations, nominal operating voltage has been lowered from 1V in Virtex7 series (28nm) to 0.72V in Ultrascale+ series (16nm); resulting in 1.2X and 2.4X in power and performance/watt efficiency, respectively \cite{xilinx}. Also, in each technology node, supply voltage lowering below the standard nominal level can deliver further power savings. %
 However, one of the key impediments to this approach is the increase of the delay of the underlying hardware circuit when the supply voltage is lowered. Two approaches exist to tackle this issue: \textit{first}, simultaneously underscaling the voltage and frequency. This technique aims to dynamically set the most optimal voltage-frequency pair, where no timing violation is experienced, and relatively acceptable power and energy efficiency is obtained. However, its downside is the performance degradation as the consequence of the frequency lowering \cite{Semeraro2002}. \textit{Second}, the more aggressive approach is to allow the device to work in the critical regions, where the frequency is not directly decreased and thus, timing faults occur in aggressively low-voltage regions. Understanding the behavior of these faults and efficiently mitigate them can deliver further power and energy savings in low-voltage designs without performance degradation. This approach was studied for multiple devices, e.g., processors \cite{vlv}; however, to the best of our knowledge, such studies have not been thoroughly undertaken for FPGAs.

More specifically, this paper emphasizes on the on-chip Block-RAMs (BRAMs) of commercial FPGAs, motivated by the key role of BRAMs in the acceleration of state-of-the-art applications and also their significant contributions in the total power consumption, such as Neural Network with $\sim$30\% of such a contribution \cite{dnn}. In other words, we only undervolt BRAMs, while other components of the FPGA work at their default nominal-voltage levels. Hence, %
\textbf{the main goal of this paper} is to experimentally characterize the bit-level behavior of faults with undervolting commercial-FPGA BRAMs, below the standard nominal level. Understanding this behavior can be useful for exploring better trade-offs between the FPGA energy, power, performance, and/or reliability in aggressively low-voltage scenarios. %
 \textit{To the best of our knowledge, this is the first work to perform such detailed study for aggressively reducing supply voltage for commercial FPGAs.} 
Our experiments are performed on two Xilinx FPGA platforms with 28nm technology. Through BRAM undervolting of these platforms, we observed that that data can be safely retrieved without any observable fault until a certain, $V_{min}$, which implies the existing of a voltage guardband. %
Further undervolting below $V_{min}$, causes faults in some locations of some BRAMs, with an exponentially increasing fault rate of up to 0.06\%. %
 The main contributions of this work is summarized as follows:
\begin{itemize}
\item We perform the first detailed experimental bit-level characterization study of the behavior of faults at below $V_{min}$ regions. More specifically, we observe that: 
\begin{itemize}
\item The fault rate exponentially increases by further undervolting. These faults mostly manifest themselves as stuck-at-0 bit flips, with a non-uniform distribution over various BRAMs. 
\item Bits that are corrupted in a certain level of supply voltage are remained faulty at lower voltages, as well. It is called Fault Inclusion Property (FIP) that was observed for cache structure of processors \cite{Gottscho2014}. We are the first to experimentally observe and characterize the FIP property for FPGAs.
\item In higher environmental temperatures, the fault rate decreases. This behavior is the result of the Inverse Temperature Dependence (ITD) \cite{Neshatpour2018}, which states that in nanometer technology nodes, the propagation delay is reduced in higher temperature environments that in turn, leads in a lower fault rate.
\end{itemize}
\item We empirically show that by exploiting the built-in ECC in BRAMs, more than 90\% of these faults are covered, with a negligible power overhead of ECC activation. This efficiency is the consequence of the single-bit nature of these faults, which in fact fits the capability of built-in ECC that has the type of Single-Error Correction and Double-Error Detection (SECDED).%
\end{itemize}

This paper is organized as follows. In Section II we introduce the experimental setup. The overall behavior of BRAM unvervolting is described in Section III. Fault characterization and mitigation are discussed in Section IV and Section V, respectively. %
In Section VI we review the previous work, and finally Section VII concludes and summarizes the paper. 

==> Camera-Ready-5pages_arXiv/chapters/4-methodology.tex <==
\section{Experimental methodology}
\begin{table}[!t]
\caption{Specifications of Tested Platforms.}
\label{table:spec}
\centering
\begin{tabular}{|c|c|c|}
\hline
\textbf{Hardware Platform (Board)}                            & VC707                & KC705                \\ \hline \hline
\textbf{Device Family} & Virtex 7 & Kintex 7 \\ 
\textbf{Chip Model}                       & XC7VX485T          & XC7K325T             \\ 
\textbf{Number of BRAMs}                  & 2060                 & 890                  \\ 
\textbf{Basic Size of Each BRAM}          & 1024*16-bits				 & 1024*16-bits				 \\ 
\textbf{Manufacturing Process Technology} & 28nm                & 28nm                \\ 
\textbf{Nominal $V_{CCBRAM}$ ($V_{nom}$)}                  & 1V                  & 1V                  \\ \hline
\end{tabular}
\end{table}

We perform our experiments on two commercial FPGA boards from Xilinx, i.e., VC707 and KC705 with Virtex7 and Kintex7 series, respectively. Their FPGAs are respectively equipped with 2060 and 890 BRAMs, distributed all over the chip with the size of 16 Kbits each. Each BRAM is a matrix of bitcells with 1024 rows and 16 columns. BRAMs can be either individually accessed or cascaded to build larger memories (with some overheads). This methodology provides flexibility for the FPGA designers to have single-cycle access to on-chip memories as per bandwidth or size needs. %
More details of our tested platforms are shown in Table \ref{table:spec}. Both platforms are fabricated with 28nm technology and the standard nominal voltage of BRAMs is the same, $V_{nom}= 1V$. However, due to their datasheet, VC707 is performance-oriented designed in contrast KC705 that is optimized for the power. Hence, for a through evaluation, we selected these representative products. %

\begin{figure}
  \includegraphics[width=\linewidth]{./images/1.png}
  \caption{An Overview of the Experimental Setup.}
  \label{fig:setup}
\end{figure}

Through the Power Management Bus (PMBUS) standard \cite{pmbus}, it is possible to independently and dynamically regulate and monitor the supply voltage of such FPGA components as BRAMs ($V_{CCBRAM}$), core logic ($V_{CCINT}$), and IOs ($V_{CCIO}$). For the implementation, we use Texas Instrument (TI) PMBUS USB Adapter, and the provided C-based Application Programming Interface (API), which facilitates to access the voltage controller through the host \cite{ti}.  %
The experimental setup is shown in Fig. \ref{fig:setup}. It is composed of two distinct hardware and software components. The task of the hardware FPGA platform is to walk on BRAMs and transmit their content to the host, using a serial interface. On the hardware design and to cross clock domains, we use a double-clock synchronization FIFO with $F_{BRAM}$ and $F_{UART}$ clocks. $F_{BRAM}$ is set to the maximum frequency that our design can operate on without any timing violation in the nominal voltage, 100Mhz. $F_{UART}$ is fixed to 50Mhz, a reliable frequency to transmit data. %
On the other side, the host issues the required PMBUS commands to set a certain voltage to $V_{CCBRAM}$. %
Also, it initializes BRAMs and analyzes faulty data retrieved from BRAMs. Note that we verify and validate that the implemented serial interface is fully reliable in any $V_{CCBRAM}$ level. On this setup, the reduced $V_{CCBRAM}$ with the initial operating frequency, $F_{BRAM}$= 100Mhz, can cause the timing violations and in turn, corruption of some of bitcells of some of BRAMs. We follow the method below to comprehensively analyze the behavior of these faults:


\fbox{\begin{minipage}{0.46\textwidth}
\textit{ \\  
1. $F_{BRAM}= F_{max}= 100Mhz$    \\  
2: $V_{CCBRAM}= V_{min}= 0.61V$;        \\
3: while($V_{CCBRAM} >= V_{crash}$ begin \\
4:\hspace*{0.5ex}\hspace{2.5ex}while(numRun $<=$ 100) begin\\
5:\hspace*{0.5ex}\hspace{2.5ex}\hspace{2.5ex}delay(1sec);                              \\
6:\hspace*{0.5ex}\hspace{2.5ex}\hspace{2.5ex}Write pattern to all BRAMs;         \\
7:\hspace*{0.5ex}\hspace{2.5ex}\hspace{2.5ex}Transfer content of BRAMs to the host;  \\
8:\hspace*{0.5ex}\hspace{2.5ex}\hspace{2.5ex}Analyse faulty data (ratio and location);     \\
9:\hspace*{0.5ex}\hspace{2.5ex}\hspace{2.5ex}numRun++;               \\
10:\hspace*{0.5ex}\hspace{2.5ex}end\\
11:\hspace*{0.5ex}\hspace{2.5ex}$V_{CCBRAM} =- 10 (mV)$;   \\
12: end
}
\end{minipage}}

In short, first, we initialize $V_{CCBRAM}$ with $V_{min}$, $F_{BRAM}$ with the maximum operating frequency 100Mhz, and BRAMs with a certain pattern. Then, retrieve the content of BRAMs one-by-one and within each BRAM row-by-row, and transfer them to the host. In the host, we analyze the ratio and location of faults. This process is repeated 100 times for a certain level of voltage to obtain statistically significant results. The reported results in this paper are the median of these 100 tests. After a soft reset, we decrease $V_{CCBRAM}$ by 10mV and repeat the process above until the lowest voltage that our design operate on, $V_{crash}$. %
Finally, to measure the power consumption with acceptable accuracy, we use Xilinx Power Estimation Tool (XPE) combined with a power meter.%




==> Camera-Ready-5pages_arXiv/chapters/5-results.tex <==



\section{Fault Characterization}
In this section, we comprehensively characterize the behavior of faults, where $V_{CCBRAM}$ is underscaled from $V_{min}= 0.61V$ to $V_{crash}= 0.54V$. As can be seen in Fig. \ref{subfig:major707} and \ref{subfig:major705}, the fault rate in VC707 is relatively more than KC705, by 47.4\% on average. This difference can be the consequence of the architectural and technological differences adopted to optimize performance and power in VC707 and KC705, respectively.

\subsection{Fault Stability Over Time} 
As earlier mentioned, we repeat each test 100 times to get statistically significant results. We did not observe a significant difference among runs, since the standard deviation of the fault rate and locations among these runs is negligible. More details about these 100 runs are summarized in Table. \ref{table:repeat}. Thus, it can be concluded that faults follow mostly a permanent (stuck-at) behavior.


\begin{table}[]
\centering
\caption{Fault Rate Stability Over Time. Fault Rate Analysis of 100 runs at $V_{crash}=0.54V$ with pattern=16'hFFFF.}
\label{table:repeat}
\begin{tabular}{|c|c|c|}
\hline
      \textbf{Parameter}                                 & \textbf{VC707} & \textbf{KC705} \\   \hline \hline
\multicolumn{1}{|l|}{\textbf{AVERAGE fault rate} (per 1 Mbit)}     & 652            & 254            \\
\multicolumn{1}{|l|}{\textbf{MINIMUM fault rate} (per 1 Mbit)}     & 630            & 240            \\
\multicolumn{1}{|l|}{\textbf{MAXIMUM fault rate} (per 1 Mbit)}     & 669            & 264            \\
\multicolumn{1}{|l|}{\textbf{STANDARD DEVIATION of fault rates}} & 7.3            & 4.8            \\ \hline
\end{tabular}
\end{table}

\begin{figure}[!t]
\centering
\subfloat[VC707]{\includegraphics[width=1.65in]{./images/81.png}%
\label{subfig:clustering707}}
\hfill
\subfloat[KC705]{\includegraphics[width=1.65in]{./images/82.png}%
\label{subfig:clustering705}}
\caption{The Impact of the Data Pattern in the Fault Rate.}
\label{fig:pattern}
\end{figure}

\begin{figure*}[!t]
  \includegraphics[width=\linewidth]{./images/28.png}
  \caption{Fault Variation Map (FVM) for VC707, scaling $V_{CCBRAM}$ from $V_{min}= 0.61V$ to $V_{crash}= 0.54V$.}
  \label{fig:fvm}
\end{figure*}

\subsection{Impact of Data Pattern}
Below the $V_{min}=0.61V$, the fault rate exponentially increases up to 652 and 254 per 1 Mbits ($\sim$ 0.06\% and 0.03\%)\footnote{Since the overall fault rates are very small, instead of percentage (\%), we present them in terms of number of faults per 1Mbit, for clearer charts.} at $V_{crash}=0.54V$, for VC707 and KC705, respectively (with pattern= 16'hFFFF). Furthermore, we observed that the vast majority of these faults are "1" to "0" bit flips, on average 99.9\%. We verify this observation by repeating the same tests with other data patterns. As shown in Fig. \ref{fig:pattern}, the fault rate is proportional to the number of "1" bits; for example, with pattern= 16'hFFFF the fault rate is almost double than pattern= 16'hAAAA, and with pattern=16'h0000 few faults are observed. In the same line, we did not observe any meaningful correlation in the various permutations of "0" and "1" in the data pattern, for instance, as can be seen, the fault rate of pattern= 16'hAAAA, 16'h5555, and a random pattern are almost the same. In short, through our experiments, faults in aggressively low-voltage regions manifest themselves as stuck-at-0 bit flips. Considering the behavior as mentioned above, we present the rest of results in this section, for the data pattern= 16'hFFFF. 





\subsection{Fault Variability Among and Within BRAMs}
This section describes our observations on fault variability among and within BRAMs.
\subsubsection{BRAM-to-BRAM Fault Variation} 
By statistically analyzing experimental results, we observed that the fault rates in aggressively low-voltage regions below $V_{min}=0.61V$ considerably varies among BRAMs. For instance, experimenting on VC707 at $V_{crash}=0.54V$, the maximum, minimum, and average fault rate within BRAMs are 2.84\%, 0\%, and 0.04\%, respectively. Also, 38.9\% of BRAMs in VC707 and 45.2\% in KC705 has no observable faults. As a further analysis, we clustered this statistical information in low-, mid-, and high-vulnerable classes of BRAMs, using the k-means clustering algorithm. As can be seen in Table.  \ref{table:clustering}, for instance, the vast majority of BRAMs in VC707, 88.6\%, are recognized as low-vulnerable with an average fault rate of 0.02\%, $\sim$ 3.4 faults within an individual BRAM with the size of 1024*16-bits. 


\begin{table}[]
\centering
\caption{Clustering BRAMs due to Vulnerability Features (Reported numbers are at $V_{crash}= 0.54V$).}
\label{table:clustering}
\begin{tabular}{cl|l|l|}
\cline{3-4}
\multicolumn{1}{l}{}                                                                     &                         & \textbf{VC707} & \textbf{KC705} \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{67FD9A}}                                           & \%BRAMs                 & 88.6\%         & 93.4\%         \\
\multicolumn{1}{|c|}{\multirow{-2}{*}{\cellcolor[HTML]{67FD9A}\textbf{low-vulnerable}}}  & Average Fault Rate (\%) & 0.02\%         & 0.01\%         \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFE65}}                                           & \%BRAMs                 & 9.4\%          & 5.7\%          \\
\multicolumn{1}{|c|}{\multirow{-2}{*}{\cellcolor[HTML]{FFFE65}\textbf{mid-vulnerable}}}  & Average Fault Rate (\%) & 0.24\%         & 0.17\%         \\ \hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{FE0000}}                                           & \%BRAMs                 & 1.8\%          & 0.9\%          \\
\multicolumn{1}{|c|}{\multirow{-2}{*}{\cellcolor[HTML]{FE0000}\textbf{high-vulnerable}}} & Average Fault Rate (\%) & 0.86\%         & 0.74\%         \\ \hline
\end{tabular}
\end{table}

\begin{figure}[!t]
\centering
\subfloat[Column Vulnerability Within Individual BRAMs.]{\includegraphics[width=1.65in]{./images/70.png}%
\label{subfig:vul1}}
\hfill
\subfloat[Column Vulnerability Averaged Over BRAMs.]{\includegraphics[width=1.65in]{./images/71.png}%
\label{subfig:vul2}}
\caption{Fault Variability Within BRAMs for VC707, at $V_{crash}=0.54V$. (Very Similar Results with KC705)}
\label{fig:vul}
\end{figure}

\begin{figure*}[!t]
\centering
\subfloat[On-board Temperature= 50$^\circ$C]{\includegraphics[width=1.65in]{./images/31.png}%
\label{subfig:t50}}
\hfill
\subfloat[On-board Temperature= 60$^\circ$C]{\includegraphics[width=1.65in]{./images/32.png}%
\label{subfig:t60}}
\hfill
\subfloat[On-board Temperature= 70$^\circ$C]{\includegraphics[width=1.65in]{./images/33.png}%
\label{subfig:t70}}
\hfill
\subfloat[On-board Temperature= 80$^\circ$C]{\includegraphics[width=1.65in]{./images/34.png}%
\label{subfig:t80}}
\caption{The correlation among on-board temperature, supply voltage of BRAMs, technology (VC707 vs. KC705), and fault rate. (x-axis: $V_{CCBRAM}$ from $V_{min}= 0.61V$ to $V_{crash}= 0.54V$, y-axis: the fault rate (per 1Mbit))}
\label{fig:temperature}
\end{figure*}

 This significant fault variability among BRAMs can be due to either the chip-dependent process variation or design tools for place and route. We verify this argument by performing the following test; for our test design, we extracted the fault rate of BRAMs with several place-and-route compiles. Repeating the voltage lowering operation on these various bitstreams, we observed almost an identical fault rate in the corresponding physical locations of BRAMs. Hence, we conclude that this fault rate variability among BRAMs is the result of the process variation. According to this test and also the permanent behavior of faults, as earlier explained, we construct a chip-dependent Fault Variation Map (FVM). FVM is extracted by mapping the observed fault rates to the physical location of BRAMs on the tested chips. Through Vivado, Xilinx design compiler, we extract the required information to build FVM, including the floorplan of the chip and the placement information of BRAMs. For instance, FVM of VC707 is shown in Fig. \ref{fig:fvm}, when $V_{CCBRAM}$ is lowered from $V_{min}=0.61V$ to $V_{crash}=0.54V$. FVM has the granularity of BRAM. Note that in this figure other FPGA components are ignored for the sake of more clarity. The chip-dependent property of FVM provides an opportunity to optimize the FPGA-based designs. 



\begin{figure}[!t]
  \includegraphics[width=\linewidth]{./images/91.png}
  \caption{Fault Inclusion Property (FIP), undervolting BRAMs from $V_{min}=0.61V$ to $V_{crash}=0.54V$, shown for VC707. (FIP is a verified on KC705, as well.)}
  \label{fig:fip}
\end{figure}


\subsubsection{Within-BRAM Fault Variation}
We performed a statistical analysis to analyze the fault distribution schema within those faulty BRAMs. Our observations reveals that faults mostly occur in a few certain columns within BRAMs. In other words, for each faulty BRAM, a few (one or two) most vulnerable column of bitcells exist, among 16 available columns. Fig. \ref{subfig:vul1} shows the number of most vulnerable columns within faulty BRAMs. As can be seen, more than 80\% of faults occur in a single column, 17\% in two columns, and so on. However, these most vulnerable columns do not occur in identical column indexes, for different BRAMs. As can be seen in Fig. \ref{subfig:vul2}, there is almost a uniform distribution of fault rate in different 16 available column indexes, when fault rate is averaged for all BRAMs.     
 


\subsection{Fault Inclusion Property (FIP)} 
Fault Inclusion Property (FIP) is a property that we experimentally observed by monitoring the fault location and rate under various supply voltages below $V_{min}=0.61V$. FIP is said to exist if all the faulty bits in a certain level of $V_{CCBRAM}$ are still faulty in further reduced levels of voltage. FIP was previously observed for CPU cache structures \cite{Gottscho2014}, here we confirm that FIP holds for FPGA on-chip memories as well, as visualized in Fig. \ref{fig:fip}. While it may not be the best representation as the figure shows the stacked fault rates; however, through our experimental results we observed both location as well as rate of faults in a certain voltage level are exactly repeated in lower voltage levels. Also, FIP in the BRAM-level can be seen in the FVM of Fig. \ref{fig:fvm}. 



 \begin{table*}[]
\centering
\caption{Summary of Fault Characterization in FPGA-Based BRAMs and comparing with the modern DRAMs.}
\label{table:FaultSummery}
\begin{tabular}{|
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l |
>{\columncolor[HTML]{FFFFFF}}l |}
\hline
\multicolumn{1}{|c|}{\cellcolor[HTML]{FFFFFF}\textbf{Key Finding}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{BRAM {[}our work{]}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{DRAM \cite{Chang2017}}} \\ \hline \hline
Below $V_{nom}$ and above $V_{min}$, no observable fault.                  & $V_{nom}= 1V, V_{min}= 0.61V$                                                     & $V_{nom}= 1.5V, V_{min}= 1.25V$                                             \\ \hline
Type of faults: Permanent                                                   & Stuck-at-0                                                     & Stuck-at-0 and stuck-at-1                                                 \\ \hline
Impact of data pattern.   & Fault ratio is directly related to number of "1" logic.    & Fault ratio is independent of the pattern.    \\ \hline
Below $V_{min}$, fault ratio \textit{exponentially} increases.                 & Valid, chip-dependent, on average {[}0,$\sim$0.06\%{]}                            & Valid, vendor-dependent, on average {[}0, $\sim$20\%{]}                    \\ \hline
Faults tends to cluster in certain locations.                    & Certain BRAMs                                                             & Certain Banks                                                       \\ \hline
Fault Inclusion Property (FIT) & Follows this property. & Is not discussed.\\ \hline
Temperature has a linear effect on the fault ratio.                                            & Higher temperature leads in \textit{less} faults.                                  & Higher temperature leads in \textit{more} faults.                            \\ \hline
\end{tabular}
\end{table*}







\subsection{Impact of the Environmental Temperature}
We perform an experiment to study the effect of the environmental temperature on the behavior of faults when $V_{CCBRAM}$ is dropped below $V_{min}$. Toward this goal, we repeat the original design described in Section II, while the hardware platform is placed inside a chamber that its temperature can be regulated by a heater. In this setup, we underscale the $V_{CCBRAM}$ and retrieve the content of BRAMs to extract the fault rate, while controlling and monitoring the on-board temperature in the host, through an on-chip sensor. The experimental results are shown in Fig. \ref{fig:temperature} under various on-board temperatures, 50$^\circ$C (default temperature), 60$^\circ$C, 70$^\circ$C, and 80$^\circ$C. As can be seen, with heating up, the fault rate is constantly reduced. For instance, the fault rate reduces by more than 3X for the VC707, by going from the default on-board temperature, 50$^\circ$C to 80$^\circ$C. This observation is the consequence of the Inverse Thermal Independence (ITD) property \cite{Neshatpour2018}. ITD is a thermal property of devices with nanoscale technology nodes. It states that in contrast with the traditional CMOS technologies, in the nanoscale technology nodes at low-operating voltages the circuit delay reduces. The reason is that as the technology scales down, the supply approaches the threshold voltage. Hence, at low-voltage regimes, increasing the temperature reduces the threshold voltage and allows the device to switch faster at higher temperatures. With the circuit delay decrease, subsequently, the number of critical paths, and in turn, the rate of timing faults in the critical paths are reduced, as we experimental verified in our case. %
 Also, as can be seen, the fault rate in VC707 is reduced more aggressively than KC705. A relatively 156\% more fault rate in 50$^\circ$C is reduced to 11.6\% less ratio in 80$^\circ$C, for VC707 vs. KC705. The architectural and technological difference between these platforms can be the reason, since their design goal is different; performance (VC707) and power (KC705).








\subsection{Summary}
We presented comprehensive fault characterization results under BRAM undervolting below $V_{min}$. Our experimental observations such as stuck-at-0 behavior of faults and significant fault rate variability among BRAMs, can provide an opportunity to optimize power-reliability trade-offs in aggressively low-voltage regimes, for applications implemented onto FPGAs. We summarize our observations and findings in Table. \ref{table:FaultSummery}. Also, we compare our observations with a recent characterization work on DDR-3 \cite{Chang2017}, mostly in the behavioral-level. Although, there is a technological difference between them, i.e., BRAMs are SRAM-based while DDR-3 are DRAM-based, the comparison highlights their significant similar fault behavior under low-voltage operations.













==> Camera-Ready-5pages_arXiv/chapters/7-dnn.tex <==
\section{FPGA-based Neural Network (NN) Acceleration on Low-voltage BRAMs}
In this section, we present and discuss the results of our study on the impact of the BRAM voltage scaling below nominal level, $V_{nom}=1V$, in a typical FPGA-based NN application. More specifically, our study includes the power consumption and NN accuracy trade-off, and an efficient fault mitigation technique for operating below $V_{min}=0.61V$. We perform our experiments on a fully-connected NN in the inference phase on MNIST dataset \cite{mnist}. MNIST is an image recognition benchmark suite, working on black and white digitized handwritten digits, each image 784*8-bit pixels, the output infers the number from 0 to 9. This model is composed of input, hidden, and output layers, where all neurons of adjacent layers are fully connected to each other. The intensity of each connection is determined by weights. The first layer is called input layer, and it has one neuron for each component in the input vector (e.g., each pixel). The last layer is called output layer and contains one neuron for each component in the output vector (e.g., each output class). Between the input and output layers, there are hidden layers. The interconnection between neurons of adjacent layers is determined based on a collection of weights and biases, whose values are tuned in the training phase. Each neuron of the NN uses an activation function (typically logarithmic sigmoid) to quantize its output. Finally, in the output layer, a softmax function generates the final output of the NN. The softmax function determines the probability distribution of the input vector over all different possible outcomes. Typically, NNs encompass two distinct phases; training and inference (classification/prediction/recognition). The training is a one-time process to determine weights and biases, which is usually performed off-line. In contrast, the inference phase repeatedly runs to classify unknown data. In this paper, we study the inference phase of the given NN. Hence, weights and biases of neurons are imported from an off-line training phase. 



\begin{table}[]
\centering
\caption{Specifications of our FPGA-based NN Experimental Setup.}
\label{table:nnsetup}
\begin{tabular}{|l|l|}
\hline
\multicolumn{2}{|c|}{\textbf{Neural Network}}                                                 \\ \hline \hline
\textbf{Type}                       & Fully-Connected Classifier                  \\ 
\textbf{Topology (\#layers)}        & 6L (1L input, 4L hidden, 1L output)                     \\ 
\textbf{Size per Layer (\#neurons)} & (784, 1024, 512, 256, 128, 10)= 2714                    \\ \
\textbf{\#Weights}                  & $\sim$1.5 million                                      \\ 
\textbf{Activation Function}        & Logarithmic Sigmoid                                     \\ \hline \hline
\multicolumn{2}{|c|}{\textbf{Data Representation Model}}                                      \\ \hline \hline
\textbf{Type}                       & 16-bits fixed point                                     \\ 
\textbf{Precision}                  & Min sign and digit per layer (Fig. \ref{fig:precision})              \\ \hline \hline
\multicolumn{2}{|c|}{\textbf{Benchmark}}                                                      \\ \hline \hline
\textbf{Name-Type}                  & MNIST \cite{mnist}- Handwritten Digits \\ 
\textbf{\#Images}                   & Training: 60000, Inference: 10000                  \\ 
\textbf{\#Pixels per Image}         & 28*28= 784                                              \\ 
\textbf{\#Classes}                  & 10                                                      \\ \hline \hline
\multicolumn{2}{|c|}{\textbf{FPGA Implementation}}                                            \\ \hline \hline
\textbf{FPGA Platform-Chip}              & VC707-Virtex7 (Table I)                                                   \\ 
\textbf{Operating Frequency}        & 100Mhz                                                  \\ 
\textbf{BRAM Usage} (Total: 2060)   & 70.8\%                                                  \\
\textbf{DSP Usage} (Total: 2800)    & 58.3\%                                                  \\ 
\textbf{FF Usage} (Total: 303,600)  & 13.1\%                                                  \\ 
\textbf{LUT Usage} (Total: 607,200) & 43.1\%                                                  \\ \hline
\end{tabular}
\end{table}

\subsection{Introducing the Experimental Setup of NN Evaluating}
Detailed specifications of our experimental setup are summarized in Table \ref{table:nnsetup}. In our system architecture, weights of the NN are located inside BRAMs and input images are being streamed through the off-chip DDR-3. The required calculation of the image classification, matrix multiplication plus sigmoid function activation, are performed in parallel by leveraging  DSPs and LookUp Tables (LUTs) of the FPGA and results are streamed to the host computer to perform the final step of the NN accuracy analysis. This is a typical setup for most of the FPGA-based NN accelerator, as surveyed in \cite{dnn}. In this section, we present results for VC707 platform since a very similar efficiency is observed for KC705. 

\begin{figure}
  \includegraphics[width=0.9\linewidth]{./images/44.png}
  \caption{Minimum Precision to Represent Weights of NN.}
  \label{fig:precision}
\end{figure}

Due to the existing constraint on the number of BRAMs in VC707, our tested NN has a 6-layers topology, i.e., ($\{L_i, i \in [0,5]\}$), composed of one input,  four hidden, and one output layer(s). Sizes of these layers are 784, 1024, 512, 256, 128, and 10, respectively. Thus, there are five set of weights, i.e., ($\{Layer_j, j \in [0,4]\}$), where $Layer_j$ refers to the weight set between $L_j$ and $L_{j+1}$. This setting leads to $\sim$1.5 million weights, which fills more than 70.8\% BRAMs in the FPGA of VC707 platform. The matrix multiplications, comprising of multiply-accumulate operations, are performed in parallel and streaming-fashion to achieve significant performance. The maximum operating frequency of our design is 100Mhz and the area utilization is summarized as 58.3\%, 13.1\%, and 43.1\% for DSP, FF, and LUT, respectively.    

The training phase of the NN is performed off-line using 60000 training images, by a MATLAB implementation. For the image classification, we first export weights and biases of the trained NN, initialize BRAMs with these parameters, and repeat the classification of 10000 images at various levels of $V_{CCBRAM}$. Also, for representing data, we use the fixed-point low-precision model. Note that lowering the precision of data is a common technique for applications in the approximate computing domain, such as NN especially in the inference stage \cite{fpgafp} and multimedia \cite{alvarez}, to achieve power and performance efficiency with negligible accuracy loss. Following these studies, we use per-layer minimum precision fixed-point model for weights. The bit-width of weights is fixed to 16-bits, composed of the sign, digit, and fraction components. Toward this goal, with a pre-processing analysis, we extract the minimum bit-widths of the sign and digit components per layer. As can be seen in Fig. \ref{fig:precision}, except the last layer, $Layer_4$, weights of other layers are in (-1, 1) margin, which means that there is no need for the digit component. However, for the $Layer_4$, a 4-bit digit component is used, the minimum width to represent data without any NN accuracy loss.     

\begin{figure}
  \includegraphics[width=0.9\linewidth]{./images/62.png}
  \caption{BRAM Power Savings of our FPGA-based NN at $V_{nom}, V_{min},$ and $V_{crash}$.}
  \label{fig:dnnpower}
\end{figure}

\begin{figure}
  \includegraphics[width=0.9\linewidth]{./images/41.png}
  \caption{Impact of BRAM Voltage Scaling in the NN Classification Error, lowering $V_{CCBRAM}$ from $V_{min}=0.61V$ to $V_{crash}= 0.54V$.}
  \label{fig:dnncharacterization}
\end{figure}

\begin{figure*}
\centering
  \includegraphics[width=\linewidth]{./images/60.png}
  \caption{Methodology of our Mitigation Technique in FPGA-based NN, Intelligently-Constrained BRAM Placement (ICBP).}
  \label{fig:overalldnn}
\end{figure*}

On this setup, the BRAM power consumption in various $V_{CCBRAM}s$ at $V_{nom}=1V$, $V_{min}=0.61V$, and $V_{crash}=0.54V$, is shown in Fig. \ref{fig:dnnpower}. %
As can be seen, more than an order of magnitude BRAM power dissipation is reduced from $V_{nom}=1V$ to the guardband gap on $V_{min}=0.61V$. Further voltage lowering to $V_{crash}=0.54V$, reduces 40\% of BRAM power over $V_{min}=0.61V$; however, as a result of the timing faults, the NN classification error is in turn impacted. This impact and the proposed fault mitigation technique are discussed later in this section.%

\subsection{The Impact of BRAM Voltage Scaling Below $V_{min}$ on the FPGA-based NN Accelerator}
When $V_{CCBRAM}$ is underscaled in the critical region between $V_{min}= 0.61V$ and $V_{crash}= 0.54V$, faults occurring in some of BRAMs bitcells degrade the NN accuracy. In fact, the classification error is increased from 2.56\% (inherent classification error without any fault) to 6.15\% when $V_{CCBRAM}= V_{crash}= 0.54V$, see Fig. \ref{fig:dnncharacterization}. The NN classification error (left y-axis) increases exponentially, correlated directly with the fault rate increase in BRAMs (right y-axis), as expected. 

Furthermore, we observe that the fault rate in BRAMs filled with the NN weights is significantly less than the default pattern= 16h'FFFF. The reason is that weights are sparse, our statistical analysis indicates that 76.3\% of the bits having the logic value '0'. These bits have a negligible probability to be flipped, especially considering that most of the timing faults in the critical low voltage operation are stuck-at-0. This experimentally verified failure characteristic is the reason that MNIST application on our NN is inherently fault-tolerant against faults in extremely low-voltage operations on FPGA-based BRAMs. Note that other state-of-the-art has also confirmed the sparsity of many other NN benchmarks \cite{minerva}, \cite{moons}, which would indicate that those applications would be inherently fault-tolerant for the type of failures experienced in FPGA BRAM undervolting.      

\subsection{Proposed Fault Mitigation Technique in FPGA-based NNs: Intelligently-Constrained BRAM Placement (ICBP)}
The overall methodology of the proposed fault mitigation technique, Intelligently-Constrained BRAM Placement (ICBP), is shown in Fig. \ref{fig:overalldnn}. It can be used for low-voltage regions below $V_{min}=0.61V$. The key motivation is that low-voltage operations dramatically reduce power consumption (for our case, 40\% in $V_{crash}=0.54V$ over $V_{min}=0.61V$); however, cause faults, which, in turn, leads to NN accuracy loss (for our case, 3.59\% additional NN classification error in $V_{crash}=0.54V$). The objective is to achieve this power-savings without significant impact on the NN classification error. 

\subsubsection{Elaborating the Proposed ICBP Algorithm}
The proposed technique relies on two key observations:
\begin{itemize}
\item \encircle{1} As detailed in Section II, we observed that faults occurred in reduced voltage BRAMs have deterministic and chip-dependent behavior. So once we have the fault map, we can exploit it to mitigate faults. Also, there is significant fault variability among BRAMs, as exposed with some BRAMs having relatively low-vulnerability as the Fault Variability Map (FVM) demonstrates in Fig. 7.
\item \encircle{2} We observed that various layers of the given NN have different inherent vulnerability to faults. We conducted a pre-processing analysis and observed that inner layers (layers closer to the output) are relatively more vulnerable, as similarly observed in \cite{layers}, \cite{dnnfault} since faults in these layers have relatively less probability to be masked through the quantification and thresholding in the activation functions.
\end{itemize}

Due to these observations, ICPB introduces a simple yet effective BRAM placement algorithm that maps the weights of the inner NN layers to low-vulnerable BRAMs, targeting to mitigate faults and achieve power-savings with minimized NN classification accuracy loss (\encircle{3}). Note that FPGAs are uniquely suited to benefit from ICBP. In comparison, CPU´s have inherent disadvantages that make it challenging to apply aggressive undervolting ideas such as ICBP for their on-chip memories due to two reasons: \textit{First}, it is extremely difficult, if not impossible to construct the undervolting fault map for CPU on-chip memories such as caches. \textit{Second}, it is very cumbersome, if not impossible, to reconfigure and remap application data into cache regions that have low vulnerability.

\begin{figure}
  \includegraphics[width=0.9\linewidth]{./images/61.png}
  \caption{Statistical Analysis of NN Layers: Size (\#BRAMs), \#Faults (at $V_{crash}=0.54V$), and Normalized Vulnerability.}
  \label{fig:layers}
\end{figure}

For further analysis, we present detailed statistical information of the different layers of the given NN, i.e., the size (in terms of utilized number of BRAMs to locate weights of the corresponding NN layer), number of faults, and the normalized vulnerability of the individual layers, as shown in Fig. \ref{fig:layers}. As can be seen, outer layers (closer to the input layer) are relatively larger, which experience more faults, as expected. Note that by statistical analysis, we observed that outer layers are relatively more sparse; thus, the per-layer fault rate is not exactly proportional to the per-layer size; however, both size (number of BRAMs) and number of faults show an exponential behavior among various layers. Also, it is important to note that we conducted a software-based statistical fault injection campaign to extract the vulnerability of various NN layers. As can be seen, for instance, $Layer_5$ is around 6X more vulnerable than the first one, $Layer_0$, which means that the same rate of faults injected in $Layer_4$ causes 6X NN classification error than injecting the same number of faults in $Layer_0$. The conclusion of analyzing different NN layers is that inner layers are significantly smaller, relatively less probable to experience faults; however, those inner layers are the most vulnerable layers where each fault has much more impact on the quality of the result, in turn means that they need more protection. 


\subsubsection{Implementation Methodology}
As earlier noted, in ICBP we aim to constrain the BRAM placement algorithm to map the logical BRAMs of inner NN layers to low-vulnerable physical BRAMs in the chip. Note that logical BRAMs are defined in the high-level verlog design description and in contrast, physical BRAMs refers to the BRAM locations in the FPGA. Toward this goal, we exploit the Physical Blocks (Pblocks) facility of Vivado, a Xilinx implementation tool. Pblocks provides a fully flexible facility to constrain logical blocks, e.g., BRAMs, to a physical region in the FPGA. As described in Section II, we classify physical BRAMs into low-, mid-, and high-vulnerable classes. Having the list of physical locations of these BRAMs (XY), we first, create corresponding low-, mid-, and high-vulnerable Pblocks and then, appropriately assign the logical BRAMs into these Pblocks.  

\begin{figure}[!t]
\captionof{List}{Illustrating Pblock Creation and BRAM Assignement for FPGAs. \label{list:pblock}}
\fbox{\begin{minipage}[t]{0.48\textwidth}
\textbf{1:} \textit{create\_pblock} low-vulnerable\_pblock \\\underline{\textbf{\%Creation of a Pblock, low-vulnerable\_pblock}}\\
\textbf{2:} \textit{resize\_pblock} [get\_pblocks low-vulnerable\_pblock] -add \{RAMB18\_X0Y44 RAMB18\_X3Y91 RAMB18\_X1Y26\} \\\underline{\textbf{\%Assigning 3 physical BRAMs to low-vulnerable\_pblock}}\\
\textbf{3:} \textit{add\_cells\_to\_pblock} [get\_pblocks low-vulnerable\_pblock] [get\_cells -quiet [list \{l-BRAM[0]\}\{l-BRAM[1]\}]] \\\underline{\textbf{\%Assigning 2 logical BRAMs to low-vulnerable\_pblock}}
\end{minipage}}
\end{figure}

The example in List. \ref{list:pblock} illustrates the creation and BRAM assignment of Pblocks using TCL commands. This example creates a Pblock (low-vulnerable\_pblock), assigns three physical BRAMs in locations (X0Y44, X3Y91, and X1Y26), and adds two logical BRAMs (l-BRAM[0] and l-BRAM[1]). This is a post-synthesize constraint that is added to the Xilinx Design Constraints (XDC) file. In consequence, the placement tool of Vivado will try to find the most efficient placement of these two logical BRAMs into the specified three physical BRAM locations. By following this methodology, we create our three low-, mid-, and high-vulnerable Pblocks, each includes the corresponding physical BRAMs specified by our fault characterization. Fig. \ref{subfig:pblock} shows a schematic of the created Pblocks in VC707 platform. As expected, the low-vulnerable\_pblock is dominating since it involves 88.6\% of physical BRAMs. Also, the effect of ICBP in the final implementation of the design can be seen by comparing its schematic view in Fig. \ref{subfig:intelligentplacement} with the default placement (without any Pblock constraint) in Fig. \ref{subfig:defaultplacement}. Note that Fig. \ref{subfig:intelligentplacement} refers to the design that all logical BRAMs of our design including all weights (not only the inner layers) are forced to be located in low-vulnerable BRAMs. As expected, the default placement results in more compacted design since the low-vulnerable BRAMs are distributed all over the chip, which limits ICBP to make a more compacted design. This specific design increases the timing slack by 50\% over the default placement. However, as earlier noted, we aim to locate only inner layers of the NN into low-vulnerable BRAMs, which can eliminate this overhead, thanks to their significantly smaller sizes of inner layers. Later in this section, we discuss this trade-off and different aspects of ICBP. 
 
\begin{figure}[!t]
\centering
\subfloat[Schematic of Low-, Mid-, and High-vulnerable Pblocks.]{\includegraphics[width=1.15in]{./images/64.png}%
\label{subfig:pblock}}
\hfill
\subfloat[The Schematic of the Proposed ICBP in our NN Design.]{\includegraphics[width=1.05in]{./images/66.png}%
\label{subfig:intelligentplacement}}
\hfill
\subfloat[The schematic of the Default Placement in our NN Design.]{\includegraphics[width=1.05in]{./images/65.png}%
\label{subfig:defaultplacement}}
\caption{Pblocks and its Impact in the Schematic of the NN Design Placement in VC707 Platform.}
\label{fig:pblock}
\end{figure}

\subsubsection{Experimental Results}
We evaluate several variations of the proposed mechanism, where "ICBP-N" refers to a version of ICBP that the last N layers of the NN are located in low-vulnerable BRAMs, $N \in \{1,2,3,4,5\}$. For instance, "ICBP-1" version means that weights of the "only last layer", i.e., $Layer_4$, are forced to be located in low-vulnerable BRAMs, while a normal BRAM placement is applied to the other layers. In the same line, "ICBP-5" version means that all layers, i.e., ($\{Layer_j, j \in [0,4]\}$) are located in low-vulnerable BRAMs, as its schematic placement is shown in Fig. \ref{subfig:intelligentplacement}. In Fig. \ref{subfig:mitigResults}, we compare the impact of different BRAM placement techniques in the NN classification error when $V_{CCBRAM}=V_{crash}=0.54V$, i.e., \textit{i}) default BRAM placement, \textit{ii}) different variations of the proposed BRAM placement technique, ICBP-N, $N \in \{1,2,3,4,5\}$, and \textit{iii}) the worst-case placement where the inner NN layers are located in the high-vulnerable BRAMs, the rest in mid-, and low-vulnerable BRAMs in order. As can be seen, the classification error is decreased from 6.1\% with the default placement to 3.01\% in "ICBP-1" version, where only $Layer_4$ is forced to leverage low-vulnerable BRAMs. Note that $Layer_4$ is the smallest among the NN layers and most sensitive layer to faults, thus, its protection significantly prevented the NN accuracy loss. By intelligently placing additional layers, the classification error is further decreased and reduces to 2.6\%, which is very close to the inherent classification error of 2.56\%.     

However, since the low-vulnerable BRAMs are distributed all over the chip, ICBP may incur the timing overhead, as reported in Fig. \ref{subfig:mitOverhead} in terms of the percentage of the timing slack increase over the default placement. As can be seen, the timing slack is significantly increased in the more aggressive versions and reaches to 50\% in "ICBP-5", where all NN layers are located in low-vulnerable BRAMs. However, for "ICBP-1" this overhead is negligible since a very small number of BRAMs, two BRAMs, are forced to exploit the low-vulnerable BRAMs.        

\begin{figure}[!t]
\centering
\subfloat[Classification Error of NN Impacted by Faults with Different BRAM Placements at $V_{crash}=0.54V$.]{\includegraphics[width=0.9\linewidth]{./images/47.png}%
\label{subfig:mitigResults}}
\hfill
\subfloat[Timing Slack Overhead of ICBP-N.]{\includegraphics[width=0.9\linewidth]{./images/48.png}%
\label{subfig:mitOverhead}}
\caption{Evaluating our Fault Mitigation Technique, ICBP.}
\label{fig:mitigFinal}
\end{figure}

We repeat our most effective and timing cost-free version of the proposed mitigation technique, "ICBP-1", by lowering $V_{CCBRAM}$ from $V_{min}=0.61V$ to $V_{crash}=0.54V$, to explore the optimal voltage level in terms of power consumption and NN classification error trade-off, as shown in Fig. \ref{fig:tradeoff}. As can be seen in Fig. \ref{subfig:tradeoff1}, 40\% power savings is achieved in $V_{crash}=0.54V$ over $V_{min}=0.61V$, by 0.6\% NN accuracy loss from the inherent fault-free classification error of 2.56\%; however, the same amount of power in the default placement is dissipated by more than 3.59\% NN accuracy loss. 

Since $V_{CCBRAM}$ scaling inversely impacts power consumption, and NN classification error, we aim to find the optimal voltage level as the best trade-off. Toward this goal, experimental results are analyzed in terms of a new metric, the normalized product of power consumption with NN classification error, as shown in Fig. \ref{subfig:optimal}. As can be seen, \textit{first}, due to this trade-off $V_{CCBRAM}=0.56V$ is the optimal voltage level for "ICBP-1", which leads to 28.1\% of power saving achievements over the $V_{min}=0.61V$, while the classification error increase up to 2.66\% (0.1\% overhead from the inherent fault-free classification error, 2.56\%). \textit{Second}, the efficiency of "ICBP-1" technique in comparison to the default placement technique, is relatively better manifested in lower levels of $V_{CCBRAM}$ since in relatively higher voltage levels, the fault rate and its subsequent impact on the NN accuracy is not considerable.               

\begin{figure}[!t]
\centering
\subfloat[Power Reduction and NN Classification Error.]{\includegraphics[width=0.9\linewidth]{./images/63.png}%
\label{subfig:tradeoff1}}
\hfill
\subfloat[The Optimal $V_{CCBRAM}$, Trading-off Power and NN Accuracy.]{\includegraphics[width=0.9\linewidth]{./images/67.png}%
\label{subfig:optimal}}
\caption{"ICBP-1" Mitigation on Various $V_{CCBRAM}s$ in [$V_{min}=0.61V, V_{crash}=0.54V$].}
\label{fig:tradeoff}
\end{figure}

\subsection{Summary and Discussion on the Methodology and Results}
We summarize our findings on power and resilience trade-off in low-voltage FPGAs, as follows:

\textit{-- Power:} Our experimental results on real hardware identified a significant potential in commercial FPGAs to operate in low-voltage regimes below standard level and in turn, to work in ultra low-power modes. For a NN test application, we showed the BRAM power savings of more than an order of magnitude by voltage lowering until $V_{min}$ and a further 40\% below $V_{min}$. It is obvious that the overall power saving gains depends on the contribution of BRAMs in the corresponding design. For instance, in our evaluated NN accelerator, in total 25.8\% of the total power is decreased, due to 28.2\% BRAMs contribution in the total power consumption. However, with similar voltage underscaling on other power-hungry components of the design, such as off-chip DDR-3, DSPs, and LUTs, we expect to achieve further power saving gains. For instance, a recent study on low-voltage operations of DDR-3 \cite{Chang2017} reported 10.5\% energy-savings, which can be combined with our design to further save the total power dissipation. 

\textit{-- Resilience:} Although, we observed that in FPGA-based BRAMs the fault rate below $V_{min}$ increases exponentially, they can be efficiently mitigated. Toward an efficient mitigation two observations play key role; \textit{first}, the characterization of fault behavior, and \textit{second}, the inherent resilience features of the application against faults. By combing these two observations in our FPGA-based NN, the impact of faults is minimized to 0.1\% with significant power savings of 28.1\%. It is important to note that this paper focused on one of the main observed behaviors of faults, significant variability among BRAMs. However, we think that there is untapped existing potential in leveraging other findings in our study such as stuck-at-0 type of faults, BRAM fault distribution, etc.        








==> Camera-Ready-5pages_arXiv/chapters/9-setup.tex <==
\section{Experimental Methodology}
We perform our experiments on two FPGAs, i.e., XC7VX485T representing the Virtex7 family on a VC707 board and XC7K325T representing the Kintex7 series on a KC705 board. These FPGAs are respectively equipped with 2060 and 890 BRAMs, distributed over the chip with the size of 16 Kbits each. Each BRAM is a matrix of bitcells with 1024 rows and 16 columns. BRAMs can be either individually accessed or cascaded to build larger memories (with some overheads). This methodology provides flexibility for the FPGA designers to have single-cycle access to on-chip memories as per bandwidth or size needs. %
More details of our tested platforms are shown in Table \ref{table:spec}. Both platforms are fabricated with 28nm technology, and the standard nominal voltage of BRAMs is the same, $V_{nom}= 1V$. However, their difference is that XC7VX485T (Virtex7) is designed for performance while XC7K325T (Kintex7) is optimized for the power consumption. Hence, for a thorough evaluation, we selected these representative FPGAs. %

\begin{table}[!t]
\caption{Specifications of Tested Platforms.}
\label{table:spec}
\centering
\begin{tabular}{|c|c|c|}
\hline
\textbf{Hardware Platform (Board)}                            & VC707                & KC705                \\ \hline \hline
\textbf{Device Family} & Virtex 7 & Kintex 7 \\ 
\textbf{Chip Model}                       & XC7VX485T          & XC7K325T             \\ 
\textbf{Number of BRAMs}                  & 2060                 & 890                  \\ 
\textbf{Basic Size of Each BRAM}          & 1024*16-bits				 & 1024*16-bits				 \\ 
\textbf{Manufacturing Process Technology} & 28nm                & 28nm                \\ 
\textbf{Nominal $V_{CCBRAM}$ ($V_{nom}$)}                  & 1V                  & 1V                  \\ \hline
\end{tabular}
\end{table}

\begin{figure}
  \includegraphics[width=0.9\linewidth]{./images/90.png} %
  \caption{Experimental Setup to Perform Fault Study in FPGA BRAMs.}
  \label{fig:setup}
\end{figure}

Through the Power Management Bus (PMBUS) standard \cite{pmbus}, it is possible to independently and dynamically regulate and monitor the supply voltage of such FPGA components as BRAMs ($V_{CCBRAM}$), core logic ($V_{CCINT}$), and IOs ($V_{CCIO}$). To modify $V_{CCBRAM}$, we use Texas Instrument (TI) PMBUS USB Adapter, and the provided C-based Application Programming Interface (API), which facilitates accessing the on-board voltage controller through the host \cite{ti}.  %
The experimental setup is shown in Fig. \ref{fig:setup}. It is composed of two distinct hardware and software components. The task of the hardware FPGA platform is to access BRAMs and transmit their content to the host, using a serial interface. To cross clock domains, we use a double-clock synchronization FIFO with $F_{BRAM}$ and $F_{UART}$ clocks. $F_{BRAM}$ is set to the maximum frequency that our design can operate without any timing violation in the nominal voltage, 100Mhz. $F_{UART}$ is fixed to 50Mhz, a reliable frequency to transmit data. %
On the other side, the host issues the required PMBUS commands to set a certain voltage to $V_{CCBRAM}$. %
Also, it initializes BRAMs and analyzes potentially faulty data retrieved from BRAMs. Note that we verify and validate that the implemented serial interface is entirely reliable in any $V_{CCBRAM}$ level. On this setup, the reduced $V_{CCBRAM}$ can cause timing violations and in turn, corrupting some of bitcells of some of BRAMs. We follow the method shown in List. \ref{list:bram} to analyze the behavior of these faults comprehensively.


\begin{figure}[!t]
\captionof{List}{Pseudo-code to Study Voltage Scaling on BRAMs, on the Experimental Setup of Fig. \ref{fig:setup}. \label{list:bram}}
\fbox{\begin{minipage}{0.46\textwidth}
\textit{ \\  
1: $F_{BRAM}= F_{max}= 100Mhz$;    \\  
2: $V_{CCBRAM}= V_{min}= 0.61V$;        \\
3: while($V_{CCBRAM} >= V_{crash}$) begin \\
4:\hspace*{0.5ex}\hspace{2.5ex}while(numRun $<=$ 100) begin\\
5:\hspace*{0.5ex}\hspace{2.5ex}\hspace{2.5ex}delay(1sec);                              \\
6:\hspace*{0.5ex}\hspace{2.5ex}\hspace{2.5ex}Write pattern to all BRAMs;         \\
7:\hspace*{0.5ex}\hspace{2.5ex}\hspace{2.5ex}Transfer content of BRAMs to the host;  \\
8:\hspace*{0.5ex}\hspace{2.5ex}\hspace{2.5ex}Analyse faulty data (rate and location);     \\
9:\hspace*{0.5ex}\hspace{2.5ex}\hspace{2.5ex}numRun++;               \\
10:\hspace*{0.5ex}\hspace{2.5ex}end\\
11:\hspace*{0.5ex}\hspace{2.5ex}$V_{CCBRAM} =- 10 (mV)$;   \\
12: end
}
\end{minipage}}
\end{figure}

As can be seen in List \ref{list:bram}, first, we initialize $V_{CCBRAM}$ with $V_{min}=0.61V$, $F_{BRAM}$ with the maximum operating frequency $F_{max}=100Mhz$, and BRAMs with a certain pattern. Then, we retrieve the content of BRAMs one-by-one and within each BRAM row-by-row, and transfer them to the host. In the host, we analyze the rate and location of faults. This process is repeated 100 times for each voltage level to obtain statistically significant results. The reported results in this paper are the median of these 100 tests. After a soft reset, we decrease $V_{CCBRAM}$ by 10mV and repeat the process until the lowest voltage that our design operate, $V_{crash}=0.54V$. %
Finally, to measure the power consumption with acceptable accuracy, we use Xilinx Power Estimation Tool (XPE) combined with a power meter. It is important to note that since we perform our experiments without frequency scaling of the given design, the achievements on the power ratios are equivalent to the energy savings. %



==> Camera-Ready-5pages_arXiv/subfloat/Makefile <==
SUBFLOATDIR=subfloat
INSTALLDIR=`kpsewhich --expand-path='$$TEXMFLOCAL'`/tex/latex/subfloat
DOCDIR=`kpsewhich --expand-path='$$TEXMFLOCAL'`/doc/latex/subfloat
VERSION=`grep '^\\\\def\\\\fileversion' subfloat.dtx | sed 's/^\\\\def\\\\fileversion{\\(.*\\)\\.\\(.*\\)}/\\1_\\2/'`

.SUFFIXES: .sty .ins .dtx .dvi .ps


.ins.sty:
	latex $<

.dtx.dvi:
	latex $<
	latex $<
	makeindex -s gind.ist $(*D)/$(*F)
	makeindex -s gglo.ist -o $(*D)/$(*F).gls $(*D)/$(*F).glo
	latex $<

.dvi.ps:
	dvips -o $(*D)/$(*F).ps $(*D)/$(*F)


all: subfloat.sty subfloat.dvi ausgabe 

subfloat: subfloat.sty

clean:
	@-rm -f subfloat.{glo,gls,idx,ilg,ind,aux,log,toc}
	@-rm -f *~

distclean: clean
	@-rm -f subfloat.{sty,dvi,ps}

tar:	all clean
	echo Lege subfloat.tar.gz an
	-rm -f subfloat-*.tar.gz
	tar czCf .. subfloat-$(VERSION).tar.gz \
	  $(SUBFLOATDIR)/README $(SUBFLOATDIR)/Makefile \
	  $(SUBFLOATDIR)/subfloat.{dtx,ins,dvi} \
	  $(SUBFLOATDIR)/install.sh \
	  $(SUBFLOATDIR)/subfloat.xml $(SUBFLOATDIR)/ChangeLog

zip:	all clean
	-@rm -f subfloat-$(VERSION).zip
	mkdirhier tex/latex/subfloat
	mkdirhier doc/latex/subfloat
	mkdirhier source/latex/subfloat
	mv subfloat.sty tex/latex/subfloat
	cp subfloat.{dtx,ins,xml} Makefile source/latex/subfloat
	cp ChangeLog README subfloat.dvi doc/latex/subfloat
	zip -r subfloat-$(VERSION).zip tex doc source
	rm -r tex/ doc/ source/

install: all
	if [ ! -d $(INSTALLDIR) ]; then mkdirhier $(INSTALLDIR); fi
	if [ ! -d $(DOCDIR) ]; then mkdirhier $(DOCDIR); fi
	install -m622 subfloat.sty $(INSTALLDIR)
	install -m622 subfloat.dvi $(DOCDIR)
	texhash

ausgabe:
	@echo "Please copy subfloat.sty to a directory"
	@echo "in the LaTeX search path"

tpm:	all
	mkdirhier texmf-local/tex/latex/subfloat
	mkdirhier texmf-local/doc/latex/subfloat
	mkdirhier texmf-local/source/latex/subfloat
	cp subfloat.dtx subfloat.ins README Makefile texmf-local/source/latex/subfloat
	cp README subfloat.dvi texmf-local/doc/latex/subfloat
	cp subfloat.sty texmf-local/tex/latex/subfloat
	@-rm -f subfloat.zip
	zip -r subfloat texmf-local
	rm -rf texmf-local



subfloat.sty: subfloat.ins subfloat.dtx



